Verification of Neural Networks Local Differential Classification Privacy

Neural networks are susceptible to privacy attacks. To date, no verifier can reason about the privacy of individuals participating in the training set. We propose a new privacy property, called local differential classification privacy (LDCP), extending local robustness to a differential privacy setting suitable for black-box classifiers. Given a neighborhood of inputs, a classifier is LDCP if it classifies all inputs the same regardless of whether it is trained with the full dataset or whether any single entry is omitted. A naive algorithm is highly impractical because it involves training a very large number of networks and verifying local robustness of the given neighborhood separately for every network. We propose Sphynx, an algorithm that computes an abstraction of all networks, with a high probability, from a small set of networks, and verifies LDCP directly on the abstract network. The challenge is twofold: network parameters do not adhere to a known distribution probability, making it difficult to predict an abstraction, and predicting too large abstraction harms the verification. Our key idea is to transform the parameters into a distribution given by KDE, allowing to keep the over-approximation error small. To verify LDCP, we extend a MILP verifier to analyze an abstract network. Experimental results show that by training only 7% of the networks, Sphynx predicts an abstract network obtaining 93% verification accuracy and reducing the analysis time by $1.7\cdot10^4$x.

==> alg_old.tex <==
\section{Prediction of an Interval Hyper-Network}
\label{sec:alg}

In this section, we introduce \tool's algorithm for predicting an interval hyper-network, called \alg.
We begin by describing the algorithm and then provide details.
\alg takes as inputs a network $N$, a training algorithm $\mathcal{T}$, a training set $\mathcal{D}$, and a probability error bound $\alpha$, where $\alpha \in (0,1)$ is a small number (e.g., $\alpha=0.05$).
It returns an interval hyper-network $\mathcal{N}^\#$ which, with probability $1-\alpha$ (under certain conditions), provides an abstraction of $N$ and every concrete network returned by $\mathcal{T}$ given $\mathcal{D}\setminus\{(x,y)\}$, for every entry $(x,y)\in\mathcal{D}$.
The main idea is to predict an abstraction for every network parameter from a small number of concrete networks.
To minimize the number of networks,
\alg executes iterations.
An iteration trains a few networks and predicts an interval hyper-network from all networks.
If the coverage of the new hyper-network is improved compared to the previous iteration, another iteration begins.
We next outline the algorithm, then provide details, and finally
discuss correctness.

\paragraph{\alg's algorithm}
\Cref{alg:gen} shows the algorithm of \alg.
It begins by initializing the set of trained networks \texttt{nets} to $N$ and the set of entries \texttt{entr}, whose corresponding networks are in \texttt{nets}, to $\emptyset$.
It initializes the previous hyper-network $\mathcal{N}^\#_{prev}$ to $\bot$ and the current hyper-network $\mathcal{N}^\#_{curr}$ to the interval abstraction of $N$, i.e., the interval of a network parameter $w\in \mathcal{W}\cup\mathcal{B}$ (a weight or a bias) is $[w^N,w^N]$.
Then, while the stopping condition, comparing the coverage of $\mathcal{N}^\#_{prev}$ and $\mathcal{N}^\#_{curr}$ (as described shortly), is \texttt{false}, it runs an iteration.
An iteration trains $k$ new networks~(\Cref{ln:trbegin}--\Cref{ln:trend}).
A training iteration samples an entry $(x,y)$, adds it to \texttt{entr}, and runs the training algorithm $\mathcal{T}$ on the architecture of $N$ and $\mathcal{D}\setminus\{(x,y)\}$.
The trained network is added to \texttt{nets}.
\alg then computes an interval hyper-network from \texttt{nets}~(\Cref{ln:abbegin}--\Cref{ln:abend}).
The computation is executed via \intalg (\Cref{sec:algpredict}) independently on each network parameter $w$.
\intalg's inputs are all observed values of $w$ and a probability error bound $\alpha'$, which is $\alpha$ divided by the number of unseen networks multiplied by the number of network parameters.
%We describe \intalg in~\Cref{sec:algpredict}.
%Afterwards, \alg checks a stopping condition, evaluating the hyper-network's interval coverage~(\Cref{ln:stop}).
%This coverage is compared to the coverage of the previous hyper-network.
%If it has not changed significantly, \alg completes and returns the last interval hyper-network.
%Otherwise, \alg continues to another iteration.
%We describe the stopping condition in~\Cref{sec:algacc}.

\begin{algorithm}[t]
\caption{\alg($N$, $\mathcal{T}$, $\mathcal{D}$, $\alpha$)}
\label{alg:gen}
\DontPrintSemicolon
\KwIn{a network $N$, a training algorithm $\mathcal{T}$, a training set $\mathcal{D}$, an error bound $\alpha$.}
\KwOut{an interval hyper-network.}
$\text{nets}\gets\{N\}$\;
$\text{entr}\gets\emptyset$\;
$\mathcal{N}^\#_{prev}\gets\bot$\;
$\mathcal{N}^\#_{curr}\gets N^\#$\;
\While{$\text{stopping\_cond}(\mathcal{N}^\#_{prev},\mathcal{N}^\#_{curr})=\text{false}$}
{\label{ln:stop}
$\mathcal{N}^\#_{prev}\gets \mathcal{N}^\#_{curr}$\;
\For{$k$ iterations}
{\label{ln:trbegin}
$(x,y)\gets\text{Random}\left(\mathcal{D}\setminus\text{entr}\right)$\;
$\text{entr}\gets\text{entr}\cup\{(x,y)\}$\;
$\text{nets}\gets\text{nets}\cup\left\{\mathcal{T}\left(N,\mathcal{D}\setminus\{(x,y)\}\right)\right\}$\;
}\label{ln:trend}
\For{$w\in\mathcal{W}\cup\mathcal{B}$}
{\label{ln:abbegin}
$\mathcal{V}_w\gets\{w^{N'} \mid N'\in\text{nets}\}$\;
$w^{\mathcal{N}^\#_{curr}}\gets\intalg\left(\mathcal{V}_w,\frac{\alpha}{(|\mathcal{D}|+1-|\text{nets}|)\cdot (|\mathcal{W}\cup \mathcal{B}|)}\right)$\;
}
}\label{ln:abend}
\Return $\mathcal{N}^\#_{curr}$\;
\end{algorithm}

\paragraph{Stopping condition}
The goal of \alg's stopping condition is to identify when the hyper-network $\mathcal{N}^\#_{curr}$ covers every concrete network, seen and unseen, with a probability of $1-\alpha$.
%The challenge is to identify when the predicted interval hyper-network provides a (sound) abstraction, which is affected by the training algorithm, the network architecture, and the training set.
To this end, it compares the two last hyper-networks $\mathcal{N}^\#_{prev}$ and $\mathcal{N}^\#_{curr}$ and checks how much the intervals expanded.
Formally, for each network parameter $w$, it computes the interval's expansion rate.
Given the previous and current intervals of $w$, $I_{prev}=[l_{prev},u_{prev}]$ and $I_{curr}=[l_{curr},u_{curr}]$, the expansion rate is:
\begin{equation*}
  e=\frac{|I_{curr}\setminus I_{prev}|}{|I_{prev}|}=\frac{\max\{u_{prev},u_{curr}\}-\min\{l_{prev},l_{curr}\}}{u_{prev}-l_{prev}}-1
\end{equation*}
By this definition, the minimal value of $e$ is 0, which is when $I_{curr}$ is contained in $I_{prev}$, namely the interval of $w$ has not expanded in the last iteration.
The condition compares $e$ to a threshold $t(k)$, which is a function of the number of networks trained at a single iteration $k$.
Intuitively, the higher the $k$ the higher the $t(k)$, thereby expressing that we expect more expansion to justify training additional networks.
If the number of network parameters above $t(k)$ is below a threshold $p_e\cdot|\mathcal{W}\cup\mathcal{B}|$ (e.g., $p_e=0.1$), then the condition is true and \alg terminates.
Namely, if most network parameters have not expanded substantially, then the stopping condition (heuristically) infers that the hyper-network $\mathcal{N}^\#_{curr}$ provides an abstraction with a probability of $1-\alpha$.

\subsection{Prediction of an Interval for a Network Parameter}
\label{sec:algpredict}
In this section, we explain how \intalg predicts an interval for a network parameter $w$ from a (small) set of values $\mathcal{V}_w=\{w_1,\ldots,w_{K}\}$, obtained from the concrete networks, and given an error bound $\alpha'$.
If we followed the standard interval abstraction, $w$ would be mapped to the interval defined by the minimum and maximum values in $\mathcal{V}_w$.
However, this approach cannot guarantee to abstract the unseen concrete networks, because there is no known probability distribution for the network parameters and since we aim to rely on a number of concrete networks smaller by few orders of magnitudes than $|\mathcal{D}|$.
Instead, \intalg's goal is to predict the minimum and maximum of $w$, over all its values in the (seen and unseen) networks and accordingly define the interval.
There has been an extensive work on estimating statistics,
 with a high probability, of an unknown probability distribution (e.g., expectation~\cite{valid_adapt,prevent_false,stab_adapt,general_adapt,pres_adapt,adapt_median,emp_adapt,limit_general}).
However, \intalg requires to estimate the minimum and maximum of unknown samples from an unknown probability distribution.
The main challenge is that, unlike other statistics, the minimum and maximum are highly sensitive to outliers.
To cope, \intalg transforms the unknown probability distribution of $w$ into a known one and then predicts the minimum and maximum to define an interval.
Before the transformation, \intalg normalizes the values in $\mathcal{V}_w$.
Overall, \intalg's operates as follows (\Cref{fig:alg_flow}):
(1)~it normalizes the values in $\mathcal{V}_w$, (2)~it transforms the values into a known probability distribution,
(3)~it predicts the minimum and maximum, with a probability of $1-\alpha'$, and (4)~it inverses the transformation and normalization to fit the original scale.
We note that executing normalization and transformation and then their inversion does not result in any information loss, because they are bijective functions.
%the normalization and transformation we use are unbounded monotonically increasing functions 
We next provide details.

\begin{figure}[t]
    \centering
    \include{alg_flow}
    \caption{The flow of \intalg for predicting an interval for a network parameter.}
    \label{fig:alg_flow}
\end{figure}

\paragraph{Transformation and normalization}
%To rely on the above bounds, \intalg requires a CDF.
%One option is to assume a density function, e.g., a Gaussian distribution, whose parameters are predicted using maximum likelihood estimation (MLE).
%However, we experimentally observe that the common density functions do not capture the distributions observed in practice.
%Thus, such assumption either leads to a very high over-approximation error or too narrow (unsound) abstraction.
%Instead, \intalg \emph{transforms} the unknown distribution into a known distribution.
%The transformation makes the random variables look as if drawn from a known probability distribution, which can then be used to predict the bounds.
\intalg transforms the values in $\mathcal{V}_w$ to make them seem as if drawn from a known probability distribution.
It employs the Yeo-Johnson transformation~\cite{transform}, which allows the input random variables to take any real value.
This transformation has a parameter $\lambda$, whose value is determined using maximum likelihood estimation (MLE), and is defined as follows:
\[
    T_\lambda(z) =
\left\{
\begin{array}{lrlr}
    \frac{(1+z)^\lambda-1}{\lambda}, & \lambda\neq0,z\geq0; \phantom{check111} &
    \log(1+z), & \lambda=0,z\geq0 \\
    -\frac{(1-z)^{2-\lambda}-1}{2-\lambda}, & \phantom{11} \lambda\neq2,z<0; \phantom{check111}&
    -\log(1-z), & \phantom{11}  \lambda=2,z<0
    \end{array}
    \right\}
\]
\intalg employs several adaptations to this transformation to fit our setting better.
First, it requires $\lambda\in [0,2]$.
This is because if $\lambda<0$, the transformed outputs have an upper bound $\frac{1}{-\lambda}$
and if $\lambda>2$, they have a lower bound $-\frac{1}{\lambda-2}$.
Since our goal is to predict the minimum and maximum values, we do not want the transformed outputs to artificially limit them.
Second, the Yeo-Johnson transformation transforms into a Gaussian distribution.
Instead, we transform to a distribution given by kernel density estimation (KDE) with a Laplace kernel, which is better suited for our setting~(\Cref{sec:eval}).
We describe KDE in~\Cref{app:kde}.
Third, the Yeo-Johnson transformation operates best when given values centered around zero.
However, training algorithms produce parameters of different scales and centered around different values.
Thus, before the transformation, \intalg normalizes the values in $\mathcal{V}_w$ to be centered around zero and have a similar scale as follows: $z_i\gets\frac{w_i-\mu}{\Delta}$, $\forall i\in [K]$.
Consequently, \intalg is invariant to translation and scaling and is thus more robust to the computations of the training algorithm~$\mathcal{T}$.
There are several possibilities to define the normalization's parameters, $\mu$ and $\Delta$, each is based on a different norm, e.g., the $L_1$, $L_2$ or $L_\infty$ norm.
In our setting, a normalization based on the $L_1$ norm works best, since we use a Laplace kernel.
Its center point is $\mu=\text{median}(w_1,\ldots,w_K)$ and its scale is the centered absolute first moment: $\Delta=\frac{1}{K}\sum_{i=1}^K|w_i-\mu|$.

\paragraph{Interval prediction}
After the transformation, \intalg has a cumulative distribution function (CDF) for the transformed values: $F_{y}(v)=\mathbb{P}\{y\leq v\}$.
Next, it predicts the minimum $l_y$ and maximum $u_y$, over all concrete networks, with a probability of $1-\alpha'$.
%Assume that the probability distribution of $W$ is known.
%We denote by $w_i$ the random variable corresponding to the parameter $W$ in the $i^\text{th}$ concrete network.
%That is, $w_i$ is a random variable with a known cumulative distribution function (CDF): $F_{w_i}(w)=\mathbb{P}\{w_i\leq w\}$.
To this end, it treats the possible values of $y$ as random variables
$y_1,\ldots,y_n$ and assumes they are independent and identically distributed (IID), where $n=|\mathcal{D}|+1$.
The first $K$ random variables are known, so the number of unknown variables is $n'=n-K$.
The goal is to predict an interval $[l_y,u_y]$ such that: $\mathbb{P}\left\{\bigwedge_{i=K+1}^{n} y_i\in[l_y,u_y]\right\}=\left(F_y(u_y)-F_y(l_y)\right)^{n'}\geq 1-\alpha'$.
This induces a closed-form solution for $[l_y,u_y]$, however it involves heavy computations.
%$l_W=F_W^{-1}\left(\frac{1-(1-\alpha)^{\frac{1}{n}}}{2}\right)$ and $u_W=F_W^{-1}\left(\frac{1+(1-\alpha)^{\frac{1}{n}}}{2}\right)$.
Instead, \intalg relies on a looser condition on $[l_y,u_y]$ which is more computationally efficient.
It is defined by the complementary probability and the union bound:
\begin{flalign*}
&\mathbb{P}\left\{\bigvee_{i=K+1}^ny_i\notin[l_y,u_y]\right\}\leq\sum_{i=K+1}^n\mathbb{P}\left\{y_i\notin[l_y,u_y]\right\}=&\\
&\sum_{i=K+1}^n\mathbb{P}\left\{y_i<l_y\right\}+\mathbb{P}\left\{y_i>u_y\right\}=n'\left(F_y(l_y)+1-F_y(u_y)\right)\leq\alpha'&
\end{flalign*}
This induces a closed-form solution:
$l_y=F_y^{-1}\left(\frac{\alpha'}{2n'}\right)$ and $u_y=F_y^{-1}\left(1-\frac{\alpha'}{2n'}\right)$.
Note that this condition does not require independent random variables.
Also, these bounds are asymptotically close to the tight bounds when $\alpha'\to0$.

\subsection{Analysis of \alg}
\label{sec:algcorr}
In this section, we discuss the correctness of \alg and its running time.

\paragraph{Correctness}
Our first lemma states the conditions under which \intalg computes an abstraction for the values of a single network parameter with a high probability.
\begin{lemma}
\label{lem}
Given a network parameter $w$ and an error bound $\alpha'$, if the observed values $w_1,\ldots,w_K$ are IID, the normalized values $z_1,\ldots,z_K$ are IID, and there exists $\lambda\in[0,2]$ such that  the distribution of the transformed normalized values $y_1,\ldots,y_K$ is similar to a distribution given by KDE with a Laplace kernel (using the bandwidth defined in~\Cref{app:kde}), then \intalg computes an interval abstracting $w_1,\ldots,w_{|\mathcal{D}|+1}$ with a probability of $1-\alpha'$.
\end{lemma}
The proof follows from the definitions of our computations.
We next justify our assumptions.
The first assumption is practically true because the distribution of $w_1,\ldots,w_K$ is the same.
This is because each is computed by the training algorithm $\mathcal{T}$ when given the training set without a random sample.
The second assumption is also practically true because the normalized values are also distributed the same.
The only source of dependence comes from the fact that given $K-1$ normalized samples, the last normalized sample can be inferred.
The last assumption, similar to the one in~\cite{transform}, holds in practice because, given IID samples, KDE provides a good estimation for an unknown distribution and constraining $\lambda\in[0,2]$ practically does not affect this estimation.
Note that \Cref{lem} does not make any assumption about the distribution of the observed values $w_1,\ldots,w_K$; only the transformed normalized values $y_1,\ldots,y_K$ have a known distribution.
Next, we state our main theorem:
\begin{theorem}
  Given a network $N$, a training algorithm $\mathcal{T}$, a training set $\mathcal{D}$ and an error bound $\alpha$, if the conditions of~\Cref{lem} hold and if the stopping condition evaluates to true only when every network parameter provides an abstraction with a probability of ${1-\alpha'}$, where $\alpha'=\frac{\alpha}{(|\mathcal{D}|+1-|\text{nets}|)\cdot (|\mathcal{W}\cup\mathcal{B}|)}$, then the hyper-network provides an abstraction with a probability of $1-\alpha$.
\end{theorem}
Proof follows by the union bound.
The assumption about the stopping condition is empirically justified in~\Cref{sec:eval}.
We note that our implementation omits $|\mathcal{W}\cup\mathcal{B}|$ from the dominator of $\alpha'$, because keeping it leads to very wide intervals, thereby reducing \tool's ability to verify the properties in $P$.
Even though our implementation does not have the theoretical guarantees, in practice, the hyper-networks provide an abstraction with a probability of $1-\alpha$ (for $\alpha=0.05$).

\paragraph{Running time}
The running time consists of the networks' training time and the time to compute the hyper-networks (the running time of the stopping condition is negligible).
The training time is the product of the number of networks and the execution time of the training algorithm $\mathcal{T}$.
The time complexity of \intalg is $O(K^2)$, where $K=|\texttt{nets}|$, and thus the computation of a hyper-network is: $O\left(K^2\cdot|\mathcal{W}\cup\mathcal{B}|\right)$.
Since \alg runs $\frac{K}{k}$ iterations, overall, the running time is $O\left(|\mathcal{T}|\cdot K + \frac{K^3}{k}\cdot|\mathcal{W}\cup\mathcal{B}|\right)$.
In practice, the second term is negligible, since $K$ is small.
Thus, the fewer trained networks the faster \alg is.


==> eval_app.tex <==
\section{Evaluation: Additional Statistics and Results}
\label{sec:eval_app}

In this section, we present additional statistics and results, described in~\Cref{sec:eval}.

\Cref{tab:models} provides statistics about the trained networks: the number of networks (which is equal to the size of the training set plus one), the architecture, the number of network parameters, the training time in seconds (of a single network), and the accuracy.
%All networks were trained over 20 epochs, using SGD with batch size 256 and learning rate of 0.1.
%We used Manhattan regularization with regularization coefficient $10^{-5}$.

\begin{table}[t]
\small
\begin{center}
\caption{The networks used in our experiments.}
\begin{tabular}{l@{\hspace{0.4cm}}c@{\hspace{0.4cm}}c@{\hspace{0.4cm}}c@{\hspace{0.4cm}}c@{\hspace{0.4cm}}c}
\toprule
Dataset & \#Networks & Architecture & \#Params & Training time (s) & Accuracy \\
\midrule
Adult & 32562 & $2\times5$ & 146 & 7.2 & 83.32 \\
 & & $2\times10$ & 341 & 6.8 & 83.00 \\
 & & $4\times5$ & 206 & 10.1 & 83.12 \\
\midrule
Bank & 31649 & $2\times5$ & 151 & 6.6 & 88.39 \\
 & & $2\times10$ & 351 & 6.8 & 89.78 \\
 & & $4\times5$ & 211 & 9.6 & 88.39 \\
\midrule
Credit & 21001 & $2\times5$ & 156 & 4.7 & 78.44 \\
 & & $2\times10$ & 361 & 4.5 & 82.03 \\
 & & $4\times5$ & 216 & 6.4 & 78.44 \\
\bottomrule
\end{tabular}
    \label{tab:models}
\quad
\end{center}
\end{table}

\Cref{tab:big} shows the accuracy obtained on larger networks.
It shows that the accuracy is not increased and sometimes decreases, compared to the evaluated networks.

\begin{table}[t]
\small
\begin{center}
\caption{Accuracy on larger architectures.}
\begin{tabular}{l@{\hspace{0.8cm}}c@{\hspace{0.8cm}}c@{\hspace{0.8cm}}c}
\toprule
Dataset & $10\times100$ & $15\times200$ & $20\times300$ \\
\midrule
Adult & 76.38 & 76.38 & 76.38 \\
\midrule
Bank & 88.39 & 88.39 & 88.39 \\
\midrule
Credit & 78.44 & 78.44 & 78.44 \\
\bottomrule
\end{tabular}
    \label{tab:big}
\quad
\end{center}
\end{table}

%To study the effectiveness of the stopping condition, we compare \alg to a variant that does not rely on the stopping condition and computes a hyper-network by training $K=300$ networks (which is more than the number of networks trained by \alg).
%We run this experiment for the $2\times10$ network trained for Adult, and we repeat it 100 times.
\Cref{fig:stop_hist} shows a histogram reporting the ratio of the coverage of \alg and the coverage of the variant that trains 300 networks and does not rely on the stopping condition.
%Results show that the ratio is very close to $1$ in all runs, thereby demonstrating that our stopping condition identifies properly when the hyper-network obtains a coverage with probability of $1-\alpha$, and thus it is safe to stop training more networks.

\begin{figure}[t]
      \centering
  \includegraphics[height=6cm,clip]{stop_hist}\vspace{0.5cm}
    \caption{A histogram showing the ratio of \alg's coverage and the coverage of a variant relying on 300 trained networks. The experiment ran for the $2\times10$ network, trained for Adult.}
    \label{fig:stop_hist}
\end{figure}

%\Cref{tab:traintime} reports the total training time of \tool and the optimal algorithm.
%Namely, this time consists only of the time it takes to train the networks, without any other computations or verification analysis.
%Results show that \alg enables to reduce the overall training time from days to minutes, because it requires only 1\% of all concrete networks.
%Since the verification time is negligible compared to these times (see \Cref{tab:rq3}) and since the execution time of the other computations of \tool are also negligible, this table actually shows the overall execution time of \tool and the optimal algorithm.


\section{New models}
\label{sec:new_models}
\begin{table}[t]
\small
\begin{center}
\caption{\tool (our) vs. the naive algorithm (nve).}
\begin{tabular}{l@{\hspace{0.2cm}}c@{\hspace{0.4cm}}r@{\hspace{0.2cm}}r@{\hspace{0.2cm}}r@{\hspace{0.2cm}}r@{\hspace{0.4cm}}r@{\hspace{0.2cm}}r@{\hspace{0.2cm}}r@{\hspace{0.2cm}}r@{\hspace{0.4cm}}r@{\hspace{0.2cm}}r@{\hspace{0.2cm}}r@{\hspace{0.2cm}}r}
\toprule
Dataset & Network & \multicolumn{4}{c}{Consistency} & \multicolumn{4}{c}{Robustness} & \multicolumn{4}{c}{Fairness} \\
 & & \multicolumn{2}{c}{Verify {\scriptsize{(\%)}}} & \multicolumn{2}{c}{Time (s)} & \multicolumn{2}{c}{Verify {\scriptsize{(\%)}}} & \multicolumn{2}{c}{Time (s)} & \multicolumn{2}{c}{Verify {\scriptsize{(\%)}}} & \multicolumn{2}{c}{Time (s)} \\
 & & nve & our & nve & our & nve & our & nve & our & nve & our & nve & our \\
\midrule
Adult & $2\times50$ &  &  &  &  &  &  &  &  &  &  &  &  \\
Adult & $4\times50$ &  &  &  &  &  &  &  &  &  &  &  &  \\
Adult & $2\times100$ &  &  &  &  &  &  &  &  &  &  &  &  \\

\midrule
Bank & $2\times50$ & 100 & 44 & 7.1 & 3.1 & 100 & 39 & 166 & 3.2 & 100 & 43 & 185 & 4.6 \\
\midrule
Credit & $2\times50$ & 100 & 49 & 4.7 & 3.0 & 100 & 41 & 110 & 3.0 & 100 & 47 & 113 & 3.4 \\
\bottomrule
\end{tabular}
    \label{tab:rq3}
    \end{center}
\end{table}



==> nn.tex <==
\tikzstyle{neuron} = [circle, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=white]
\tikzstyle{arrow} = [thick,->,>=latex]

\begin{tikzpicture}[node distance=2cm]

\node (i0) [neuron] {$x_{0,1}$};
\node (i1) [neuron, below of=i0] {$x_{0,2}$};
\node (h0) [neuron, right of=i0, xshift=1cm, label=above:{[0.5,1]}] {$x_{1,1}$};
\node (h1) [neuron, below of=h0, label=below:{[1,1.5]}] {$x_{1,2}$};
\node (z0) [neuron, right of=h0, xshift=1cm, label=above:{[-1,-0.5]}] {$x_{2,1}$};
\node (z1) [neuron, below of=z0, label=below:{[0.5,1]}] {$x_{2,2}$};
\node (y) [neuron, right of=z0, xshift=1cm, yshift=-1cm, label=above:{[-1,-0.5]}] {$N(x)$};

\draw [arrow] (i0) -- node[anchor=south] {$[1,2]$} (h0);
\draw [arrow] (i0) -- node[sloped, anchor=south east] {$[1,2]$} (h1);
\draw [arrow] (i1) -- node[sloped, anchor=north east] {$[1,2]$} (h0);
\draw [arrow] (i1) -- node[anchor=north] {$[-2,-1]$} (h1);
\draw [arrow] (h0) -- node[anchor=south] {$[1,2]$} (z0);
\draw [arrow] (h0) -- node[sloped, anchor=south east] {$[1,2]$} (z1);
\draw [arrow] (h1) -- node[sloped, anchor=north east] {$[1,2]$} (z0);
\draw [arrow] (h1) -- node[anchor=north] {$[-2,-1]$} (z1);
\draw [arrow] (z0) -- node[sloped, anchor=south] {$[1,2]$} (y);
\draw [arrow] (z1) -- node[sloped, anchor=north] {$[-2,-1]$} (y);
\end{tikzpicture}

